The Intrinsic Dimension of Collider Events and Model-Independent Searches in 100 Dimensions

The phase space of hadron collider events spans hundreds of dimensions, generating an intricate geometry that we are just starting to explore. The number of possible new physics signals is exponential in the number of dimensions and detecting all of them is currently impossible for any human or artificial intelligence. In this work we introduce a method to search for new physics model-independently in this high-dimensional space. It is based on the measurement of the most basic property of the manifold of collider events, its dimensionality. Our proposed technique does not suffer from a look-elsewhere effect that grows exponentially with the number of dimensions of the dataset, and by construction is insensitive to energy scale uncertainties. We illustrate its potential by finding new physics in simulated events with hundreds of phase space dimensions, taking as input single particles rather than jets. This study sets the stage for new model-independent search strategies based on global properties of collider data manifolds.

==> myPackages.tex <==
% For colors
\usepackage[dvipsnames]{xcolor}
\definecolor{unipd}{HTML}{9B0014}
\definecolor{urls}{HTML}{3187D8}
%\definecolor{urls}{HTML}{228DBF}

% For correct fonts
\usepackage[T1]{fontenc} % To switch to the T1 encoding
\usepackage{lmodern} % To switch to Latin Modern
\rmfamily % To load Latin Modern Roman and enable the following NFSS declarations.
% Declare that Latin Modern Roman (lmr) should take
% its bold (b) and bold extended (bx) weight, and small capital (sc) shape, 
% from the corresponding Computer Modern Roman (cmr) font, for the T1 font encoding.
\DeclareFontShape{T1}{lmr}{b}{sc}{<->ssub*cmr/bx/sc}{}
\DeclareFontShape{T1}{lmr}{bx}{sc}{<->ssub*cmr/bx/sc}{}

%For links
\usepackage{hyperref}
\hypersetup{
	colorlinks = true,
	linkcolor = {Salmon},
	citecolor= {urls},
	urlcolor= {MidnightBlue}
}

%For page size
\usepackage[top=2.8 cm, bottom=2.8 cm,left=2.7 cm, right=2.7 cm]{geometry}



%For chaps and sections style
\RequirePackage[sc, bf, big]{titlesec} % format for the title of the sections

%For TOC with references
\usepackage[nottoc]{tocbibind}
\usepackage{bookmark}

%For math
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amstext} 
\usepackage{xfrac}
\usepackage{latexsym}
\usepackage{slashed}
\usepackage{array}
\usepackage{braket}
\usepackage{dsfont}
\usepackage[compat=1.0.0]{tikz-feynman}
\usetikzlibrary{shapes.geometric}
\usepackage{enumerate}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{bm}
\usepackage{mathtools}
\usepackage{gensymb}
\usepackage{tensor}

% For figures
\usepackage{graphicx, rotating}
\usepackage{epstopdf}
\usepackage{epsfig}
\usepackage{caption}
\usepackage{subcaption}

% To show labels on the pdf
\usepackage{showkeys}

% Adds eq/fig/tab automatically
\usepackage[capitalise]{cleveref}

%For appendices for each chapter
\usepackage{appendix}

%To cite like [1-5]
\usepackage{cite}

%Var
\usepackage{lipsum}
\usepackage{comment}
\usepackage{scalerel}
\usepackage{multirow}
\usepackage{soul}
\usepackage{setspace}
\usepackage{xltabular}
